Detecting and Mitigating Hallucinations in Multilingual Summarisation

Hallucinations pose a significant challenge to the reliability of neural models for abstractive summarisation. While automatically generated summaries may be fluent, they often lack faithfulness to the original document. This issue becomes even more pronounced in low-resource settings, such as cross-lingual transfer. With the existing faithful metrics focusing on English, even measuring the extent of this phenomenon in cross-lingual settings is hard. To address this, we first develop a novel metric, mFACT, evaluating the faithfulness of non-English summaries, leveraging translation-based transfer from multiple English faithfulness metrics. We then propose a simple but effective method to reduce hallucinations with a cross-lingual transfer, which weighs the loss of each training example by its faithfulness score. Through extensive experiments in multiple languages, we demonstrate that mFACT is the metric that is most suited to detect hallucinations. Moreover, we find that our proposed loss weighting method drastically increases both performance and faithfulness according to both automatic and human evaluation when compared to strong baselines for cross-lingual transfer such as MAD-X. Our code and dataset are available at https://github.com/yfqiu-nlp/mfact-summ.

==> response-EMNLP-2023.tex <==
Responses and action items for EMNLP 2023: 

Reviewer 1ZfH (S - 3, E - 4):

%%% 
We thank the reviewer for acknowledging that mFACT can contribute to the NLP research community and their comments. We hope the additional experiments we conducted will ease the main soundness concerns. 

Q: For mFact, wish to see more comparison. For example, in addition to XNLI, any chance to include other baselines for comparison?

A: There are currently only a handful of established baselines dedicated specifically to multilingual faithfulness evaluation, as evidenced by the scarcity of reported alternatives in the existing literature. We are aware of a recent contribution at ACL 2023 [1], where XNLI is repurposed as an auxiliary task for faithfulness classification due to its linguistic similarity to our task. This underlines the inherent connection between Natural Language Inference (NLI) and faithfulness assessment [2]. 

We firmly believe in delineating the nuances that set NLI apart from faithfulness classification, particularly in the context of hallucination detection. NLI, while pertinent, might not holistically capture the intricate aspects of faithfulness evaluation. A specialised metric tailored to the challenges of hallucination detection is crucial for robust future research in this domain.

[1] Multilingual Summarization with Factual Consistency Evaluation. Aharoni et al., ACL 2023 Findings.
[2] Evaluating the Factual Consistency of Abstractive Text Summarization. EMNLP 2020.


%%% 

%%% 
Q: One thing wish to know is that if "averaging" is the best way to assemble the 4 model-based metrics. What if each individual metric is used to train mFact alone, will mFact beat all the metrics when they are trained alone?

A: We believe that relying on a single metric can introduce biased preference in models and a lack of diversity for captured hallucinations. In general, multiple teacher models lead to a robust, unbiased process [1, 2]. Using diverse metrics in mFACT's training helps the classifier detect various hallucination types. Inverse transfer experiments (Table 2) show promising correlations with both intrinsic and extrinsic hallucination metrics.

We conducted an additional experiment to support our argument. Rather than averaging four metrics, we individually apply single English metrics - DAE, QAFE, ENFS, and EntFA — to rank the XSum dataset and train a multilingual classifier similar to mFACT, denoted as DAE-M, QAFE-M, ENFS-M, and EntFA-M. We show the classification performance as follows,
While the faithfulness classification is not important by itself, we provide the results here to show that a reliable classifier can be trained for all of the metrics as a sanity check. 

	        Acc.	Prec.	Recall	F1
mFACT-Transfer	96	    96.34	95.56	95.95
DAE-M	        95.2	95.16	95.16	95.16
QAFE-M	        87.2	83.09	93.15	87.83
ENFS-M	        96.8	98.33	95.16	96.72
EntFA-M	        96.8	94.27	99.6	96.86

Evidently, mFACT exhibits superior performance compared to the two intrinsic metrics, while the two extrinsic metrics marginally outperform mFACT. We attribute this result to the nature of our evaluation procedure, which exclusively assesses all metrics on the constructed silver-reference dataset. Originating from XSum, the classification dataset inherently contains a greater prevalence of extrinsic errors compared to intrinsic errors [3,4]. To further validate these findings, we include these four systems in our human correlation analysis and examine their relevance to actual model-generated outputs, as discussed in the next response.

To verify our intuition that mFACT's aggregation of multiple metrics is primed to capture a wider array of hallucinations, we execute an additional inverse transfer experiment (XL-Sum Chinese -> XSum English) using classifiers trained with signals from single metrics. We chose to focus on the EntFA metric, as its classifier is the most reliable of all the examined metrics (96.86 F1). 
The results are presented below:

	      DAE↑	  QAFE↑	  ENFS↓   EntFA↑
MAD-X		83.38	69.69	16.38	95.6
mFACT-T	   *88.01* *78.78* *12.11* *96.96*
EntFA-M		83.47	68.57	15.98	95.52

From these outcomes, we observe that training the classifier with a single metric leads to inferior results across all the metrics, including the EntFA in which the EntFA-M model is specialised. We also note that even though EntFA-M can capture extrinsic hallucination well, it still has a limited ability to capture intrinsic hallucination (see weak DAE and QAFE improvements), showing the importance of assembling multiple metrics.


[1] One Teacher is Enough? Pre-trained Language Model Distillation from Multiple Teachers. Wu et al., ACL Findings 2021.
[2] Multiple Teacher Distillation for Robust and Greener Models. Ilichev et al., RANLP 2021.
[3] On Faithfulness and Factuality in Abstractive Summarization. Maynez et al., ACL 2020.
[4] Understanding Factuality in Abstractive Summarization with FRANK: A Benchmark for Factuality Metrics. Pagoni et al., NAACL 2021.

%%% 

%%% 
Q: in Table 5, is there result on the human evaluated correlation to compare mFact with the other 4 metrics?

A: To examine mFACT with four other metrics in the actual model's outputs rather than a silver-reference test set. We extend the existing results in Table 5. Using the specialised models we built (see details in the previous answer), we measured the Pearson and Spearman correlations to human annotation:

Metric  Pearson (rau)  P-val Spearman (rau)  P-value
mFACT-T	   *0.44*	   0	  *0.36*          0.01
DAE-M	    0.34	   0.01	   0.33	          0.01
QAFE-M	    0.25	   0.07	   0.29	          0.04
ENFS-M	    0.24	   0.07	   0.29	          0.04
EntFA-M	    0.35	   0.01	  *0.36*	      0.01

mFACT consistently emerges with the highest human correlation when compared to these four metrics. This observation underscores mFACT's robustness and its capacity to better correlate with human evaluations.

%%% 

%%% 

Q: "mFact is adopted in the weighted loss, which reports better Rouge in Chinese, Spanish, Vietnamese, French, but a little mixed in Hindi and Turkish." - any chance to give more discussion on the result in Table 4? Appreciate if more discussion can be provided on Hindi and Turkish language.

A: Your question is intriguing. In short, we currently lack a definitive explanation for these performance variations. However, we can suggest potential reasons for further investigation. Firstly, discrepancies could arise due to varying translation quality from the Google API across languages, impacting performance negatively for languages with lower translation quality. Secondly, mBERT's pre-training might underrepresent certain languages, leading to poorer results in our downstream task. 
Thirdly, this phenomenon could also be attributed to the nuanced disparity between the objectives of enhancing ROUGE scores and faithfulness [1,2,3] because the heuristic-based dataest construction naturally includes hallucinations in even the testing set [4]. We'll include this discussion in Section 7 for context.
  


[1] CaPE: Contrastive Parameter Ensembling for Reducing Hallucination in Abstractive Summarization
[2] Reducing Quantity Hallucinations in Abstractive Summarization
[3] Improving Factuality of Abstractive Summarization without Sacrificing Summary Quality
[4] Benchmarking Large Language Models for News Summarization

%%% 


Reviewer HygN (S - 3, E - 2):
We thank the reviewer for their comments.

%%% 
Q: The authors should compare their results with ChatGPT, as it can achieve better performance than cross-lingual transfer baselines, which will make your contribution less meaningful.

A: We firmly assert that employing ChatGPT or any analogous black-box model as a foundational reference in a scientific inquiry comes with substantial drawbacks. For example, recent research has exposed the significant variability in ChatGPT's performance over time, undermining the reproducibility of experiments [1]. Moreover, assessing a black-box model poses the challenge of data contamination, an issue of great magnitude with such data-intensive models [2, 3]. For more reasons to avoid using black-box models as baselines, we kindly refer the reviewer to a more comprehensive blog post written by one of ACL 2023 organizers, Anna Rogers [4].

With that being acknowledged, even a potent black-box LLM like ChatGPT exhibits inferiority when pitted against more compact, task-specific models. A case in point is [5]'s demonstration that ChatGPT lags behind state-of-the-art summarization models for monolingual English summarization. This disparity becomes more pronounced when assessing less commonly spoken languages [6]. As for the faithfulness of such models, recent studies demonstrated that ChatGPT is far from being hallucination-free when using English or low-resource languages as input [7], where it struggles mostly with extrinsic hallucinations [8]. The inverse transfer results we provide in Table 2 show that mFACT correlates well with both intrinsic metrics (DAE and QAFE) and extrinsic metrics (ENFS and EntFA), which are still a significant issue even for strong black-box models such as ChatGPT. 



[1] https://arxiv.org/pdf/2307.09009.pdf
[2] https://arxiv.org/pdf/2303.12767.pdf
[3] https://arxiv.org/pdf/2305.00118.pdf
[4] https://hackingsemantics.xyz/2023/closed-baselines/
[5] https://aclanthology.org/2023.findings-acl.29.pdf
[6] https://arxiv.org/pdf/2304.05613.pdf
[7] https://arxiv.org/pdf/2303.16104.pdf
[8] https://arxiv.org/pdf/2302.04023.pdf

%%% 

Q: Your pipeline for creating mFACT is too complex. It is model-based, and it need to be trained on the XSum dataset. The Google API is also needed. The authors should provide more details about the cost to dispel users' concerns.

A: We want to emphasise that we do *not* use the Google API at inference time but rather use it offline once to obtain the translated training example. We will clarify it better in our paper. As for using the XSum dataset for obtaining our metric, we believe the efforts we invest are on par with other popular metrics, e.g., the NLI-based methods we use as baselines [1, 2], which require training specialized models to evaluate faithfulness. Leveraging translation for developing datasets/resources is a common practice in cross-lingual and multilingual summarization [3], and future research with limited resources can be carried out using an open-source translator if additional adaptation is needed or use our mFACT-transfer for easily extending other languages using zero-shot cross-lingual transfer. For each language, our method has 92M characters to translate (~1000 GBP) on average. We will add these details to our paper.  

[1] https://aclanthology.org/2020.acl-main.173.pdf
[2] https://arxiv.org/pdf/1910.12840.pdf
[3] https://aclanthology.org/D19-1302/
 

Q: The weighted loss approach is not easily used to train large models. So, I don't think the mitigating hallucination method will contribute much.

A: As we established in our first answer, we believe that compact, task-specific models are also of great importance, as they achieve state-of-the-art across many tasks. In addition, there is a vast body of research aiming to fine-tune LLMs in a more cost-efficient manner. Two widely used methods for that are LoRA (Low-Rank Adaptation) [1] and its quantized version QLoRA [2]. We believe that such advances will allow researchers to use our method for LLMs as well. 

Furthermore, the weighted loss approach shows the potential to reduce hallucinations by acting as a "soft" sample selector during training. This adaptability can be extended to address other text attributes, such as bias and human preference, using an appropriate rating model. The weighted loss technique, characterised by its simplicity and effectiveness, outperforms existing benchmarks. Its ease of use, reproducibility, and lightweight nature position it as a valuable baseline for advancing research in precise multilingual summarization.

[1] https://arxiv.org/pdf/2106.09685.pdf
[2] https://arxiv.org/pdf/2305.14314.pdf

Q: Would you train different classifiers to obtain mFACT for each language, or would you directly train a multilingual classifier with mixed datasets?

A: We trained a multilingual model, as we believe this strategic choice safeguards against the risk of classifier degradation and aligns with our commitment to ensuring the robustness and adaptability of mFACT to varied languages and contexts.

### Response

Q: You have stated that "We show that state-of-the-art methods like MAD-X (Pfeiffer et al., 2020b) can improve the performance for low-resource summarisation, but also amplify hallucinations." I hope you could use some large models because your experiments are basically based on the models before 2022. And your conclusion may be true on previous models, but it may not be true on recent models. There are also many stable open-sourced models, such as LLaMA. I'd like to see you choose representative models to conduct experiments. I would raise the score again if you report such results.

A: 
First and foremost, we want to express our sincere gratitude for taking the time to read our rebuttal. Your time and attention are greatly appreciated.

We would like to clarify a potential misconception: MAD-X is *not* a standalone model; instead, it serves as an adapter-based tuning method designed to enhance cross-lingual transfer capabilities, with the flexibility to be seamlessly applied to a variety of models [1]. Previous research has demonstrated that employing MAD-X tuning can yield superior task performance compared to full model fine-tuning, particularly in the context of multilingual base models for low-resource languages in NLP [1,2]. We will provide further clarification on this matter in the paper.

To address your concern regarding the possibility of recent Large LLMs exhibiting no degradation in model faithfulness for these low-resource languages, it's worth noting that the most widely-used open-source LLMs, including those you mentioned in your comment, namely LLaMA and Alpaca, were exclusively trained on English inputs. This raises questions about their suitability for the specific task at hand, given their limited exposure to diverse language data.

Instead, we examined three multilingual LLMs

BLOOMZ-P3 [3] represents the instruction-tuned model derived from the multilingual BLOOM framework, utilizing the English P3 instruction-tuning dataset. It's important to note that we did not employ BLOOMZ-xP3, which is trained with a machine-translated P3 dataset. This decision was made to exclusively assess the cross-lingual transfer capabilities inherent to the multilingual model itself. In other words, we ensured that this model did not undergo training with summarization instructions in languages other than English.

Vicuna harnesses a dataset of 70,000 multilingual conversation-style interactions from ShareGPT to fine-tune LLaMA. It's worth mentioning that Vicuna originates from the monolingual LLaMA model. The inclusion of Vicuna in our evaluation aims to test the cross-lingual transfer potential arising from multilingual post-pretraining tuning, specifically the multilingual conversation-style tuning.

Phoenix [4] stands as the latest release, as of August 4th, 2023, in the realm of conversation-style LLMs, developed as an extension of BLOOMZ. Phoenix extends its training with an additional 267,000 and 189,000 instances of multilingual instruction and conversation data, building upon the foundation of BLOOMZ.

We selected three languages, aside from English, all of which are encompassed by BLOOMZ's pre-training and Vicuna and Phoenix's post-pretraining fine-tuning. The table below showcases the proportion of training instances in each language. Our consistent observation throughout this study has been that, for languages other than English, including those with moderate linguistic resources such as French and Spanish, the existing LLMs exhibit limited model faithfulness when applied in a cross-lingual context. This observation aligns with recent findings from the literature, which highlight the challenges LLMs face in maintaining faithfulness while generating content in low-resource languages [5,6]. This limitation represents a significant shortcoming of these models. We will add a discussion about our findings to the paper. 



| Model   | Language   | Proportion |   R-1   |   R-L   | mFACT  |
| ------- | ---------- | ---------- | ------- | ------- | ------ |
| Phoenix | English    |   58.60%   |  29.98  |  21.11  | 47.22  |
|         | French     |   2.10%    |  29.33  |  18.8   | 24.03  |
|         | Spanish    |   3%       |  15.92  |  10.65  | 18.69  |
|         | Hindi      |   1.10%   |   2.7   |   2.64  | 16.53  |
| Vicuna  | English    |      /     |  31.74  |  22.51  | 57.3   |
|         | French     |      /     |  23.82  |  15.99  | 23.02  |
|         | Spanish    |      /     |  12.92  |   7.42  | 23.68  |
|         | Hindi      |      /     |   1.3   |   1.29  | 13.53  |
| BLOOMZ  | English    |   30.03%   |  17.07  |  10.89  | 53.7   |
|         | French     |   12.9%    |  23.17  |  13.97  | 26.34  |
|         | Spanish    |   10.85%   |   8.54  |   4.64  | 27.9   |
|         | Hindi      |      /     |   8.22  |   7.8   | 12.52  |


[1] MAD-X: An Adapter-Based Framework for Multi-Task Cross-Lingual Transfer 
[2] MAD-G: Multilingual Adapter Generation for Efficient Cross-Lingual Transfer
[3] Crosslingual Generalization through Multitask Finetuning
[4] Phoenix: Democratizing ChatGPT across Languages
[5] Hallucinations in Large Multilingual Translation Models
[6] A Multitask, Multilingual, Multimodal Evaluation of ChatGPT on Reasoning, Hallucination, and Interactivity. 

Reviewer Pf1A (S - 4, E - 4):
We thank the reviewer for acknowledging that mFACT can contribute to the NLP research community and their comments.

Q: The proposed mFACT metric need lots of data samples in English for training the model, which could be lack of generalisation ability.

A: While we use 40K document-summary pairs, they can be automatically labelled by using English metrics, which achieves promising results on both our classification task, inverse-transfer verification and human evaluation. In terms of data-related costs, we are on par with other popular metrics, e.g., the NLI-based methods we use as baselines [1, 2], which require training specialised models to evaluate faithfulness in the monolingual case. Having said that, we agree that mFACT data requirements might be a limitation in some cases, and we will mention it in the "Limitations" section. 

[1] https://aclanthology.org/2020.acl-main.173.pdf
[2] https://arxiv.org/pdf/1910.12840.pdf


